Answer is All You Need: Instruction-following Text Embedding via Answering the Question

This work aims to build a text embedder that can capture characteristics of texts specified by user instructions. Despite its tremendous potential to deploy user-oriented embeddings, none of previous approaches provides a concrete solution for it. This paper offers a new viewpoint, which treats the instruction as a question about the input text and encodes the expected answers to obtain the representation accordingly. Intuitively, texts with the same (implicit) semantics would share similar answers following the instruction, thus leading to more similar embeddings. Specifically, we propose InBedder that instantiates this embed-via-answering idea by only fine-tuning language models on abstractive question answering tasks. InBedder demonstrates significantly improved instruction-following capabilities according to our proposed instruction awareness tests and instruction robustness tests, when applied to both large language models (LLMs) (e.g., llama-2-7b) and smaller encoder-based LMs (e.g., roberta-large). Additionally, our qualitative analysis of clustering outcomes, achieved by applying different instructions to the same corpus, demonstrates a high degree of interpretability.

==> 3-preliminary-letian.tex <==
For an input text $X$, a text embedder $\mathbf{Emb}(\cdot)$ is built to represent it as a $\mathbb{R}^D$ vector, where $D$ is the dimension number of the representation space. For a pair of texts $(X, X')$, the similarity between the two texts is calculated by a similarity function (generally cosine similarity) based on the two vectors,
% \jingbo{not sure if we need to spend two lines for this basic definition?}

\begin{equation*}
\centering
\small
\begin{aligned}
Sim(X, X') = \frac{\mathbf{Emb}(X) \cdot \mathbf{Emb}(X')}{\lVert \mathbf{Emb}(X)\rVert \lVert \mathbf{Emb}(X')\rVert}\\
\end{aligned}
\end{equation*} 

\noindent which represents a general semantic similarity between $X$ and $X'$. When we specify the evaluation standard of the similarity by an instruction, the similarity will be re-formalized as $Sim(X, X'|I)$ to represent the instruction-aware score. Here $I$ will influence the similarity evaluation on $(X, X')$ like ``What types of feedback are there?'' and ``How do customers like this product'' for a pair of customer reviews. How to incorporate the instruction $I$ into the calculation is the key point for further discussion. 
% \jingbo{it is important to add more than one example for the instruction $I$ here.}

\paragraph{Instructor.} \cite{instructor} is learned to represent the concatenated $I$ and $X$ and calculate the similarity as follows,
% \jingbo{shall we make it more explicit that it is $Sim(\mathbf{Emb}(I \oplus X), \mathbf{Emb}(I \oplus X')$ to reflect it is concatenation? Maybe we also want to add Instructor there so people will not confuse this definition with our proposed method.}

\begin{equation*}
\centering
\small
\begin{aligned}
Sim(X, X'|X) & = Sim(\mathbf{Emb}(I \oplus X), \mathbf{Emb}(I \oplus X'))  \\
\end{aligned}
\end{equation*} 

However, the instruction has very limited influence in this scenario and the surface form of $X$ dominates the representation space. For instance, the same $X$ with different $I$ will be mapped to very similar places, indicating only encoding the surface form. 

==> 4-method-letian.tex <==
To address the bias to the textual surface of $\mathbf{Emb}(I, X)$, we propose an alternative to encoding the representations of underlying outputs $Y = [y_1, \cdots, y_N]$ by prompting $X$ with $I$, where $N$ refers to the maximal decoding length to avoid infinite distributions. Here $\mathbf{Emb}_X(\cdot)$ and $\mathbf{Emb}_Y(\cdot)$ respectively refer to the embedders for the input texts and the output answers.
% \jingbo{What does it mean by $\mathbf{Emb}_X$ and $\mathbf{Emb}_Y$? I don't quite get the subscripts' meanings. I somehow found the definitions in 4.1 later. We need to define them when it is firstly mentioned.}

\begin{equation*}
\centering
\small
\begin{aligned}
\mathbf{Emb}_X(I, X) = \sum_{Y} P(Y|I \oplus X) \mathbf{Emb}_Y(Y) 
\end{aligned}
\end{equation*} 

\noindent where $Y$ is an underlying output from the instructed input with $P(Y|I, X)$ possibility and embedding $\mathbf{Emb}_Y(Y)$. However, this embedding requires astronomical calculations with $\mathcal{O}(|V|^N)$ probabilities and $\mathcal{O}(|V|^N)$ times of encoding, where $|V|$\footnote{$|V|$ is generally large, from $30,000$ to $50,000$.} refers to the vocabulary size. Thus, we introduce several techniques to approximate this embedding. 

\subsection{Context-free Word Embedding}

\yuwei{I am not sure the importance of mathematics here. Maybe can be moved to Appendix?}
First, we look at the $\mathbf{Emb}_Y(Y)$ term, which can be transformed as follows since mean pooling is generally applied for text embedding,

\begin{equation*}
\centering
\small
\begin{aligned}
\mathbf{Emb}_Y(Y) = \frac{1}{N}\sum_{i=1}^N \mathbf{Emb}_Y(y_i|Y)
\end{aligned}
\end{equation*} 

\noindent where $\mathbf{Emb}_Y(y_i|Y)$ indicates $y_i$ is embedded based on the $Y$ context. As $Y$ are prompted from the same instruction for comparison, we can assume that they generally share a similar context. Thus, we use $\mathbf{Emb}_Y(y_i)$ to approximate $\mathbf{Emb}_Y(y_i|Y)$, which can be done by a $|V|\times D$ vocabulary embedding $\mathbf{Emb}_V(\cdot)$ and helps us to circumvent the $|V|^N$ times of text embedding. 
Consequently, the embedding of $\mathbf{Emb}_X(I \oplus X)$ is transformed into

\begin{equation*}
\centering
\small
\begin{aligned}
& \mathbf{Emb}_X(I \oplus X) = \frac{1}{N}\sum_{Y} P(Y|I \oplus X)\sum_{i=1}^N \mathbf{Emb}_Y(y_i)
\end{aligned}
\end{equation*} 

\noindent as $y_i \in V$, we can view the summing from the vocabulary embedding $\mathbf{Emb}_V(v_j)$ terms. We first group $\mathbf{Emb}_V(v_j)$ that appears in the same position, i.e., when $y_i = v_j$. Thus, the weight on $\mathbf{Emb}_V(v_j)$ can be represented as 

\begin{equation*}
\centering
\small
\begin{aligned}
& \frac{1}{N}\sum_{i=1}^N p(y_i = v_j|I \oplus X)
\end{aligned}
\end{equation*} 

As $p(y_i = v_j|I \oplus X)$ for different $i$ are mutually independent conditioning on $I \oplus X$, the representation for the whole sentence is

\begin{equation*}
\centering
\small
\begin{aligned}
& \mathbf{Emb}_X(I, X) = \frac{1}{N}\sum_{j=1}^{|V|}\sum_{i=1}^N p(y_i = v_j|I, X) \mathbf{Emb}_V(v_j)\\
& = \frac{1}{N}\sum_j^{|V|}\sum_{i=1}^N p(y_i=v_j|I, X) e_j \\
\end{aligned}
\end{equation*} 

\noindent where $e_j$ represents $\mathbf{Emb}_V(v_j)$. This can be viewed as the sum over word embeddings weighted by the expectations of their appearance times in $Y$ divided by $N$. Consequently, we summarize the calculation for our simplified $\mathbf{Emb}_X(I, X)$ as

\begin{equation*}
\centering
\small
\begin{aligned}
& \mathbf{Emb}_X(I, X) = \sum_{j=1}^{|V|} \frac{1}{N}\mathbb{E}[\textbf{Count}(v_j|Y)] e_j \\
\end{aligned}
\end{equation*} 

\subsection{Expected Answer}
% \jingbo{Let's use the term ``Expected Answer''}

When calculating the $\mathbb{E}[\textbf{Count}(v_j|Y)]$, there remains a challenge to calculate the appearance expectation of $v_j$ in each position, $P(y_i=v_j|I,X)$. When prompting a conventional decoder, it requires to model to calculate 

\begin{equation*}
\centering
\small
\begin{aligned}
& \sum_{y_{1:i-1}} P(y_i=v_j|I,X,y_{1:i-1}) P(y_{1:i-1}) \\
\end{aligned}
\end{equation*} 

\noindent which requires a calculation for $|V|^{i-1}$ probabilities. Thus, we apply different inference and pre-training methods to approximate this distribution based on the model type. 

\paragraph{Causal Language Modeling} is applied for large language models like OPT and LLaMA-2. \letian{Add the pre-training and inference of CLM Models here.}

\paragraph{Masked Language Modeling} is applied for traditional bidirectional language models like RoBERTa. For pre-training, the answer will be fully masked and recovered by the language models by maximize the following objective,

\begin{equation*}
\centering
\small
\begin{aligned}
& P(y_i|I,X) = \textrm{Softmax}(\textrm{MLM}(m_i|I,X,M)) \\
\end{aligned}
\end{equation*} 

During the inference, we append fixed number of masks after the $(I,X)$ pair and predict the logit from each mask and use the averaged logit to calculate the final probability. 

\begin{equation*}
\centering
\small
\begin{aligned}
& P(V|I,X) = \textrm{Softmax}(\frac{1}{N}\sum_i^N \textrm{MLM}(m_i|I,X,M)) \\
\end{aligned}
\end{equation*} 

% \begin{equation*}
% \centering
% \small
% \begin{aligned}
% & P(y_i|I,X) = \textbf{MLM}(m_i|I,X,M) \\
% \end{aligned}
% \end{equation*} 

% \noindent where $M = [m_1, \cdots, m_N]$ is a series of mask tokens that are entailed after the $(I, X)$ pair. MLM directly predicts the probability distribution on the $i$-th mask from $N$ entailed masks, which efficiently represents $P(y_i|I,X)$. This approximation becomes more accurate when training on more samples. Another advantage of MLM is the [SEP] token after the masks will force the prompting to output important information while a conventional decoder might miss some information when a maximal decoding length exists. 

\subsection{Vocabulary Embedding}

We empirically explore different vocabulary embeddings for $e_i = \textrm{Emb}_V(v_i)$ in our experiments:

\paragraph{Embedding Layer} We directly embed the vocabularies by the first layer in the language model responsible for word embedding. This embedding empirical does not work well, which reflects the lack of semantic information of the representations in the first embedding layer. 

\paragraph{One-hot Embedding} We simply use the probabilistic distribution of the appearance expectation of each word in the vocabulary as the embedding. Empirical results show one-hot embeddings to work surprisingly well but relatively slow. Thus, we apply a \textbf{Inversed LM Head Transformation} to the probabilistic distribution, which is the inverse matrix of the last (biased) linear projection $W^{-1}\in \mathcal{R}^{|V|\times (D+1)}$. The projection transform the probability distribution to the last hidden state in the embedder, which can be viewed as a kind of dimension reduction and is shown to be successful by empirical results. 

% We apply two pre-training tasks to learn a encoder that produces representations of answer distributions: unsupervised last sentence recovery and supervised machine reading comprehension. 

% \paragraph{Last Sentence/Utterance Recovery} splits a paragraph (dialogue) into three parts which represent input text, instruction, and answer. In practice, the input text is the first three sentences in a document, while the instruction and the answer represent the fourth and fifth sentence. The answer is fully masked and require the encoder to recover it. This is a weak pre-training to teach the encoder to entail the instruction, which might not be an actual instruction from human's view.

% \paragraph{Machine Reading Comprehension} directly applies the context-based question answering datasets to learn instruction following. We pass the context, question, fully masked answer into the encoder and ask it to recover the answer. 

\subsection{Implementation Details}

We use RoBERTa-Large \cite{RoBERTa} as our backbone MLM model, optimized by AdamW \cite{AdamW} with an initial learning rate $1\times 10^{-5}$. The learning rate is scheduled by a cosine scheduler \cite{Cosine}. Our MRC dataset also incorporates multiple sources: RACE \cite{RACE}, MC-Test \cite{MC-Test}, DREAM \cite{DREAM}, MultiRC \cite{MultiRC}, C3 \cite{C3}, COPA \cite{COPA}, OpenBookQA \cite{OpenBookQA}, QASC \cite{QASC}, SocialiQA \cite{SocialiQA}, CosmosQA \cite{CosmosQA}, and SuperTweetEvalQA \cite{SuperTweetEval}. The batch size is set to $64$, and $3$ epochs for MRC. We exclude extractive MRC datasets because their answer does not contain implicit attributes.

==> tables/cluster.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.72}{
\begin{tabular}{l|l|ccccccccc}
\toprule
method                                                                      & model            & ArxivS2S & Reddit & 20Newsg. & FewRel & FewEvent & FewNerd & RateMyProf & Feedbacks & Avg.   \\
\midrule
\multirow{2}{*}{ST}                                                                          & e5-large-v2      & 41.05    & 57.39  & 47.94        & 54.09  & 58.49    & 36.83   & 4.31       & 15.49     & 39.45 \\
                                                                                            & instructor-large & 32.84 & \textbf{63.07} & 52.26 & 52.59 & \textbf{65.95} & 41.59 & 4.71 & 18.89 & 41.49 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (avg gen)\end{tabular}}   & llama-2-7b-chat  & 26.68    & 19.22  & 30.59        & 61.47  & 41.50    & 42.71   & 6.26       & 3.35      & 28.97 \\
                                                                            & llama-2-13b-chat & 33.19    & 28.56  & 32.65        & \textbf{67.21}  & 56.29    & 57.49   & 6.03       & 37.28     & 44.60 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (re-encode)\end{tabular}} & llama-2-7b-chat  & 25.92    & 19.49  & 27.54        & 55.91  & 36.75    & 44.02   & 0.85       & 5.27      & 26.97 \\
                                                                            & llama-2-13b-chat & 28.57    & 19.57  & 34.35        & 54.94  & 60.46    & 55.26   & 2.55       & 1.61      & 32.16 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (last ppt)\end{tabular}}  & llama-2-7b-chat  & 18.26    & 14.99  & 17.83        & 28.70  & 31.27    & 19.95   & 1.13       & 18.32     & 18.81 \\
                                                                            & llama-2-13b-chat & 21.71    & 18.43  & 24.28        & 39.48  & 47.43    & 25.33   & 1.99       & 18.21     & 24.61 \\
\midrule
\multirow{6}{*}{\model}                                              & roberta-large   & 24.96    & 39.93  & 41.93        & 60.30  & 60.41    & 49.02   & 3.53       & 27.04     & 38.39 \\
                                                                            & opt-350m         & 22.89    & 43.69  & 40.78        & 48.92  & 58.45    & 42.47   & 6.38       & 18.48     & 35.26 \\
                                                                            & opt-1.3b         & 29.48    & 45.88  & 46.45        & 54.47  & 61.49    & 46.09   & 6.15       & 20.26     & 38.78 \\
                                                                            & opt-2.7b         & 29.94    & 44.15  & 49.07        & 60.31  & 60.43    & 52.68   & 9.57       & 32.88     & 42.38 \\
                                                                            & llama-2-7b-lora  & \textbf{41.51}    & 50.00  & 51.29        & 62.52  & 63.54    & 58.59   & 17.53      & 36.78     & 47.72 \\
                                                                            & llama-2-7b       & 40.20    & 48.71  & \textbf{52.37}        & 64.59  & 57.57    & \textbf{61.52}   & \textbf{19.68}      & \textbf{43.15}     & \textbf{48.47} \\
\bottomrule
\end{tabular}}
\caption{Comparisons of \model with other fine-tuned models on clustering tasks with V-measure. Since \model fine-tunes models with only MRC tasks from the same initialization, it is directly comparable with RLHF. We experimented with $3$ aggregation methods for RLHF models. Note that for \model, we only present the best aggregation method for each model, i.e. ``avg gen'' for roberta-large and ``last ppt'' for others. All the experiments use the same instruction for each task, while there is no instructions appended for e5-large-v2.}
\label{tab:cluster}
\end{table*}

==> tables/letian_explanation.tex <==
\begin{table}
\centering
\small
\scalebox{0.83}{
\begin{tabular}{lll}
\toprule
& Label & Explanation \\
\midrule
\multirow{6}*{\rotatebox{90}{Emotion}}& Anger & enraged, irritated, angrily \\
& Fear & nervous, nervously, fright \\
& Sadness & depress, despair, Shame \\
& Joy & prosperity, Congratulations, ecstatic \\
& Love & affection, love, adore \\
& Surprise & astonished, amazed, amaz \\
\midrule
\multirow{5}*{\rotatebox{90}{Topic}}& Society \& Culture & religions, Christianity, faiths \\
& Health & medically, inflammation, thyroid \\
& Computers \& Internet & Browser, uninstall, software \\
& Business \& Finance & Craigslist, Loan, payday \\
& Family \& Relationships & girlfriends, romantic, flirt \\
\midrule
\multirow{5}*{\rotatebox{90}{Intent}}& share current location & medically, inflammation, thyroid \\
& request ride & Taxi, taxi, taxis \\
& get traffic information & motorists, congestion, traffic \\
& book restaurant & reservations, reservation, table \\
& get directions & highways, directions, Maps \\
\midrule
\multirow{8}*{\rotatebox{90}{NERD}}& attack & warfare, hostilities, battles \\
& airplane & aircraft, Aircraft, jets \\
& political party & socialists, Democrats, Party \\
& bodies of water & waterways, rivers, tidal \\
& written art & anthology, manuscript, poems \\
& education & university, college, campus \\
& scholar & scientist, physicist, theorist \\
& software & Linux, DirectX, Windows \\
\bottomrule
\end{tabular}
}
\caption{Evaluation of cluster explaining ability.} 
\label{tab:eval}
\end{table}

\begin{table}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{llc}
\toprule
Label & Explanation & F1 \\
\midrule
Anger & outraged, indignation, enraged & $48.5$ \\
Fear & sleepy, insomnia, workload & $37.4$ \\
Sadness & despair, depress, sadness & $46.6$ \\
Joy & prosperity, ecstatic, joyful & $54.4$ \\
Love & affection, adore, admiration & $29.8$ \\
Surprise & shame, ashamed, shameful & $7.7$\\
\midrule
book restaurant & reservations, reservation, table & $87.1$\\
get place details & bookstore, licensee, Trivia & $75.0$\\
request ride & Taxi, taxi, Uber & $98.1$\\
get directions & Maps, directions, highways & $94.4$\\
get traffic information & motorists, traffic, congestion & $100.0$\\
get weather & Weather, weather, forecast & $96.3$\\
share ETA & \multirow{2}*{transmit, sender, transmitting} & $72.1$\\
share current location & & $54.5$\\
search place & \multirow{2}*{chefs, Restaurant, restaurants} & $61.3$\\
compare place &  & $48.5$\\
/ & museums, galleries, pics & / \\
/ & table, tables, Table  & / \\
\bottomrule
\end{tabular}
}
\caption{Explanation of cluster center.} 
\label{tab:explain}
\end{table}

\begin{table}
\centering
\small
\scalebox{0.95}{
\begin{tabular}{llc}
\toprule
Label & Granularized Sub-Label \\
\midrule
\multirow{3}*{Anger} & outraged, indignation, enraged \\
 & disobedience, cruelty, distrust \\
 & irritated, irrit-, agitated \\
\midrule
\multirow{3}*{Science \& Mathematics} & organisms, geological, fossils \\
 & gases, oxidation, hydrogen \\
 & mathematical, geometry, algebra \\
\midrule
\multirow{3}*{get traffic information} & roadway, asphalt, roads \\
 & motorists, congestion, accidents \\
 & Traffic, -ffic, traffic \\
 \midrule
 \multirow{3}*{food} & flowering, fruit, dried \\
 & sandwiches, biscuits, snacks \\
 & flavored, flavours, sauces \\
\bottomrule
\end{tabular}
}
\caption{Our \model is able to granularize coarse-grained labels into fine-grained ones.} 
\label{tab:granularize}
\end{table}

\begin{table}
\centering
\small
\scalebox{0.95}{
\begin{tabular}{llc}
\toprule
Label & Discovered Reason \\
\midrule
\multirow{5}*{Negative Review} & technicians, confidentiality, negotiator \\
 & waiter, waitress, Serv- \\
 & restricts, malls, galleries \\
 & bedrooms, Rooms, rooms \\
 & sauces, tofu, carbohydrates \\
\midrule
\multirow{5}*{Hate Content} & mosques, religions, Muslims \\
 & niece, Nurse, daughter \\
 & LGBT, LGBTQ, -LGBT \\
 & Immigration, immigration, deported \\
 & women, feminists, Women \\
\bottomrule
\end{tabular}
}
\caption{Reason Discovering by \model.} 
\label{tab:reason}
\end{table}

==> tables/letian_tables.tex <==
% \begin{table*}
% \small
% \centering
% \scalebox{.95}{
% \begin{tabular}{llccccccccc}
% \toprule
% \multicolumn{2}{l}{\multirow{2}*{Method}} & \multirow{2}*{Emo} & \multirow{2}*{DB} & \multirow{2}*{SNIPS} & \multicolumn{2}{c}{NYT} & \multicolumn{3}{c}{IE} \\
%  & & & & & L & T & NERD & REL & EVENT \\
% \midrule
% \multirow{6}*{\rotatebox{90}{Unsup.}}& GloVe & $24.3$ & $\textbf{74.0}$ & $51.0$ & $30.8$ & - & $25.4$ & $33.8$ & $38.4$ \\
% & RoB$_{\textrm{Pool}}$ & $24.2$ & $17.6$ & $43.4$ & $25.1$ & - & $9.1$ & $10.7$ & $27.7$ \\
% & SimCSE & $36.3$ & $70.5$ & $64.0$ & $33.6$ & - & $21.8$ & $29.6$ & $35.8$ \\
% & RoB$_{\textrm{Prompt}}$ & $21.8$ & $20.2$ & $34.1$ & $17.2$ & - & $26.8$ & $20.8$ & $37.1$ \\
% & InnaTE$_{\textrm{LSR}}$ & $36.8$ & $57.4$ & $65.9$ & $66.5$ & - & $\textbf{38.8}$ & $\textbf{44.4}$ & $42.7$\\
% & InnaTE$_{\textrm{LUR}}$ & $\textbf{37.9}$ & $59.9$ & $\textbf{66.7}$ & $\textbf{61.4}$ & - & $37.2$ & $40.8$ & $\textbf{50.3}$\\
% \midrule
% \multirow{7}*{\rotatebox{90}{Sup.}}& SBERT & $29.9$ & $61.8$ & $67.6$ & $53.7$ & - & $21.4$ & $29.9$ & $35.6$ \\
% & SimCSE & $36.8$ & $74.0$ & $68.5$ & $31.1$ & - & $25.3$ & $34.4$ & $41.7$ \\
% & GTR & $30.6$ & $77.2$ & $69.0$ & $41.9$ & - & $25.9$ & $36.1$ & $39.6$ \\
% & E5 & $32.1$ & $\textbf{81.1}$ & $74.2$ & $39.9$ & - & $25.5$ & $39.6$ & $37.3$ \\
% & BGE & $41.6$ & $75.4$ & $73.9$ & $41.3$ & - & $24.9$ & $34.8$ & $38.5$ \\
% & Instructor & $37.7$ & $74.6$ & $73.6$ & $46.1$ & - & $30.0$ & $41.2$ & $\textbf{42.0}$ \\
% & InnaTE$_{\textrm{MRC}}$ & $\textbf{44.2}$ & $80.7$ & $\textbf{74.6}$ & $\textbf{61.7}$ & - & $\textbf{44.4}$ & $\textbf{53.5}$ & $41.1$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Clustering results of different embedding models.} 
% \label{tab:ps}
% \end{table*}

% \begin{table*}
% \small
% \centering
% \scalebox{.95}{
% \begin{tabular}{llccccccccccc}
% \toprule
% \multicolumn{2}{l}{Method} & Emotion & SST5 & Yahoo & DBPedia & SNIPS & MTOP & NYT-L & AMZN & NERD & REL & EVENT \\
% \midrule
% \multirow{6}*{\rotatebox{90}{Unsup.}}& GloVe & $24.3$ & $26.2$ & $38.3$ & $\textbf{74.0}$ & $51.0$ & $29.7$ & $30.8$ & $29.9$ & $25.4$ & $33.8$ & $38.4$ \\
% & RoB$_{\textrm{Pool}}$ & $24.2$ & $26.4$ & $14.4$ & $17.6$ & $43.4$ & $20.8$ & $25.1$ & $22.0$ & $9.1$ & $10.7$ & $27.7$ \\
% & SimCSE & $36.3$ & $27.3$ & $36.0$ & $70.5$ & $64.0$ & $30.6$ & $33.6$ & $30.0$ & $21.8$ & $29.6$ & $35.8$ \\
% & RoB$_{\textrm{Prompt}}$ & $21.8$ & $23.4$ & $16.9$ & $20.2$ & $34.1$ & $14.3$ & $17.2$ & $23.7$ & $26.8$ & $20.8$ & $37.1$ \\
% & InnaTE$_{\textrm{LSR}}$ & $36.8$ & $32.4$ & $49.3$ & $57.4$ & $65.9$ & $31.4$ & $66.5$ & $\textbf{39.3}$ & $\textbf{38.8}$ & $\textbf{44.4}$ & $42.7$\\
% & InnaTE$_{\textrm{LUR}}$ & $\textbf{37.9}$ & $\textbf{32.5}$ & $\textbf{51.0}$ & $59.9$ & $\textbf{66.7}$ & $\textbf{32.0}$ & $\textbf{61.4}$ & $37.9$ & $37.2$ & $40.8$ & $\textbf{50.3}$\\
% \midrule
% \multirow{7}*{\rotatebox{90}{Sup.}}& SBERT & $29.9$ & $29.3$ & $27.1$ & $61.8$ & $67.6$ & $36.2$ & $53.7$ & $32.7$ & $21.4$ & $29.9$ & $35.6$ \\
% & SimCSE & $36.8$ & $34.4$ & $47.1$ & $74.0$ & $68.5$ & $31.4$ & $31.1$ & $33.0$ & $25.3$ & $34.4$ & $41.7$ \\
% & GTR & $30.6$ & $27.4$ & $31.2$ & $77.2$ & $69.0$ & $34.2$ & $41.9$ & $37.8$ & $25.9$ & $36.1$ & $39.6$ \\
% & E5 & $32.1$ & $38.8$ & $39.4$ & $\textbf{81.1}$ & $74.2$ & $35.4$ & $39.9$ & $35.6$ & $25.5$ & $39.6$ & $37.3$ \\
% & BGE & $41.6$ & $\textbf{42.8}$ & $44.8$ & $75.4$ & $73.9$ & $\textbf{40.3}$ & $41.3$ & $36.5$ & $24.9$ & $34.8$ & $38.5$ \\
% & Instructor & $37.7$ & $35.2$ & $42.5$ & $74.6$ & $73.6$ & $35.5$ & $46.1$ & $38.8$ & $30.0$ & $41.2$ & $\textbf{42.0}$ \\
% & InnaTE$_{\textrm{MRC}}$ & $\textbf{44.2}$ & $41.2$ & $\textbf{50.1}$ & $80.7$ & $\textbf{74.6}$ & $36.4$ & $\textbf{61.7}$ & $\textbf{42.4}$ & $\textbf{44.4}$ & $\textbf{53.5}$ & $41.1$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparison of \model between traditional text embedders with small LMs in the same size as the backbone.} 
% \label{tab:ps}
% \end{table*}

% \begin{table*}
% \small
% \centering
% \scalebox{.95}{
% \begin{tabular}{l|ccccccccccc}
% \toprule
% model & ArxivS2S & Reddit & 20Newsg. & FewRel & FewEvent & FewNerd & RateMyProf & Feedbacks & Avg. \\
% \midrule
% GloVe & - & - & - & - & - & - & - & - & - \\
% RoBERTa & - & - & - & - & - & - & - & - & - \\
% SBERT & - & - & - & - & - & - & - & - & - \\
% SimCSE & - & - & - & - & - & - & - & - & - \\
% GTR & - & - & - & - & - & - & - & - & - \\
% E5 & - & - & - & - & - & - & - & - & - \\
% BGE & - & - & - & - & - & - & - & - & - \\
% Instructor & - & - & - & - & - & - & - & - & - \\
% \model & 24.96    & 39.93  & 41.93 & 60.30  & 60.41    & 49.02   & 3.53 & 27.04 & 38.39 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparison of \model with traditional text embedders with small LMs in the same size (except GloVe word vectors) as the backbone.} 
% \label{tab:ps}
% \end{table*}

==> tables/similarity.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.72}{
\begin{tabular}{l|l|ccccccc}
\toprule
                                                                            &                  & \begin{tabular}[c]{@{}c@{}}AskUbuntuRR\\ (map)\end{tabular} & \begin{tabular}[c]{@{}c@{}}SciDocsRR\\ (map)\end{tabular} & \begin{tabular}[c]{@{}c@{}}S.O.RR\\ (map)\end{tabular} & \begin{tabular}[c]{@{}c@{}}InstructSTSB\\ (spearman)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Emotion\\ (success rate)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Intent\\ (success rate)\end{tabular} & Avg   \\
\midrule
\multirow{2}{*}{ST}                                                                          & e5-large-v2      & 59.01                                                       & \textbf{83.84}                                                     & \textbf{50.60}                                                           & 0.00                                                                             & 81.43                                                                    & 18.57                                                                   & 48.91 \\
& instructor-large & \textbf{63.35} & 80.20 & 49.72 & -8.56 & 27.34 & 74.30 & 47.73 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (avg gen)\end{tabular}}   & llama-2-7b-chat  & 54.45                                                       & 73.26                                                     & 42.44                                                           & 11.54                                                                            & 83.65                                                                    & 74.94                                                                   & 56.71 \\
                                                                            & llama-2-13b-chat & 53.32                                                       & 79.58                                                     & 39.91                                                           & 13.42                                                                            & 89.25                                                                    & 50.67                                                                   & 54.36 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (re-encode)\end{tabular}} & llama-2-7b-chat  & 57.57                                                       & 76.19                                                     & 43.18                                                           & 18.61                                                                            & 78.13                                                                    & 81.61                                                                   & 59.22 \\
                                                                            & llama-2-13b-chat & 53.36                                                       & 77.80                                                     & 37.69                                                           & 16.88                                                                            & 77.86                                                                    & 66.72                                                                   & 55.05 \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}RLHF\\ (last ppt)\end{tabular}}  & llama-2-7b-chat  & 46.22                                                       & 53.07                                                     & 30.66                                                           & -0.65                                                                            & 95.68                                                                    & 7.08                                                                    & 38.68 \\
                                                                            & llama-2-13b-chat & 47.24                                                       & 55.85                                                     & 31.02                                                           & -1.94                                                                            & \textbf{98.73}                                                                    & 1.64                                                                    & 38.76 \\
\midrule
\multirow{6}{*}{\model}                                      & roberta-large   & 55.50                                                       & 73.80                                                     & 41.00                                                           & 14.81                                                                            & 90.39                                                                    & 91.77                                                                   & 61.21 \\
                                                                            & opt-350m         & 56.01                                                       & 66.87                                                     & 38.73                                                           & 7.74                                                                             & 85.97                                                                    & \textbf{93.15}                                                                   & 58.08 \\
                                                                            & opt-1.3b         & 59.09                                                       & 71.33                                                     & 43.08                                                           & 7.47                                                                             & 90.34                                                                    & 89.58                                                                   & 60.15 \\
                                                                            & opt-2.7b         & 59.94                                                       & 75.33                                                     & 41.93                                                           & 10.45                                                                            & 91.59                                                                    & 78.49                                                                   & 59.62 \\
                                                                            & llama-2-7b-lora  & 58.96                                                       & 80.04                                                     & 42.57                                                           & 22.09                                                                            & 93.81                                                                    & 82.89                                                                   & 63.39 \\
                                                                            & llama-2-7b       & 60.27                                                       & 80.61                                                     & 44.66                                                           & \textbf{22.07}                                                                            & 95.26                                                                    & 84.81                                                                   & \textbf{64.61} \\
\bottomrule
\end{tabular}}
\caption{Comparison of \model with other fine-tuned models on similarity-based tasks that include reranking (RR), sentence similarity and triplet selection. S.O. stands for StackOverflow.}
\label{tab:similarity}
\end{table*}
